TimelineKGQA: A Comprehensive Question-Answer Pair Generator for Temporal Knowledge Graphs

Question answering over temporal knowledge graphs (TKGs) is crucial for understanding evolving facts and relationships, yet its development is hindered by limited datasets and difficulties in generating custom QA pairs. We propose a novel categorization framework based on timeline-context relationships, along with \textbf{TimelineKGQA}, a universal temporal QA generator applicable to any TKGs. The code is available at: \url{https://github.com/PascalSun/TimelineKGQA} as an open source Python package.

==> libs/preamble.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% This file contains the packages that can be used in the beamer. %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Package to fonts family
\usepackage[T1]{fontenc}
% Package to accentuation
\usepackage[utf8]{inputenc}
% Package to Portuguese language
%\usepackage[brazil]{babel}
% Package to Figures
\usepackage{graphicx}
% Package for clipping
\usepackage{adjustbox}
%\usepackage{wrapfigure}
% Package for citation
\usepackage{natbib}
% Package to the colors
\usepackage{color}
% Package to the colors
\usepackage{xcolor}
% Packages to math symbols and expressions
\usepackage{amsfonts, amssymb, amsmath}
% Package to multiple lines and columns in table
\usepackage{multirow, array} 
% Package to create pseudo-code
% For more detail of this package: http://linorg.usp.br/CTAN/macros/latex/contrib/algorithm2e/doc/algorithm2e.pdf
\usepackage{algorithm2e}
% Package to insert code
\usepackage{listings} 
\usepackage{keyval}
% Package to justify text
\usepackage[document]{ragged2e}
% Package to manage the bibliography
%\usepackage[backend=biber, style=numeric, sorting=none]{biblatex}
% Package to facilities quotations
\usepackage{csquotes}
% Package to use multicols
\usepackage{multicol}
% Package to use tikz and its libraries
\usepackage{tikz}
\usetikzlibrary{er,positioning}
\usetikzlibrary{graphs,graphdrawing,quotes}
\usegdlibrary{force, layered, trees}
% Package for left aligned nested matrices
\usepackage{mathtools}
% Package for alternating color in table rows
%\usepackage{xcolor}
\definecolor{lightgray}{gray}{0.9}
\let\oldtabular\tabular
\let\endoldtabular\endtabular
\renewenvironment{tabular}{\rowcolors{2}{white}{lightgray}\oldtabular}{\endoldtabular}
\usepackage{listings}
\usepackage{array}

% Define citation alias
\defcitealias{NLP_Embeddings}{Embeddings~in~NLP}
\defcitealias{Neural_MT}{Neural~Machine~Translation}
\defcitealias{Statistical_MT}{Statistical~Machine~Translation}
\defcitealias{NLP_Pytorch}{NLP~with~PyTorch}
\defcitealias{NLP_Spacy}{NLP~with~Python~and~spaCy}
\defcitealias{DL_Pytorch}{Deep~Learning~with~Pytorch~Step~by~Step}


% Create a title page for each section
\AtBeginSection[]{
  \begin{frame}
  \vfill
  \centering
  \begin{beamercolorbox}[sep=8pt,center,shadow=true,rounded=true]{title}
    \usebeamerfont{title}\insertsectionhead\par%
  \end{beamercolorbox}
  \vfill
  \end{frame}
}
% short hyphen
\mathchardef\mhyphen="2D
\newcommand\tfidf{\mathit{tf\mhyphen idf}}

% https://pythonawesome.com/deep-learning-with-pytorch-step-by-step-a-beginners-guide/

\usepackage{libs/kbordermatrix}

%% argmin and argmax
\newcommand{\argmin}{\arg\!\min}
\newcommand{\argmax}{\arg\!\max}

\usepackage{emoji}
